HeLiOS: Heterogeneous LiDAR Place Recognition via Overlap-based Learning and Local Spherical Transformer

LiDAR place recognition is a crucial module in localization that matches the current location with previously observed environments. Most existing approaches in LiDAR place recognition dominantly focus on the spinning type LiDAR to exploit its large FOV for matching. However, with the recent emergence of various LiDAR types, the importance of matching data across different LiDAR types has grown significantly-a challenge that has been largely overlooked for many years. To address these challenges, we introduce HeLiOS, a deep network tailored for heterogeneous LiDAR place recognition, which utilizes small local windows with spherical transformers and optimal transport-based cluster assignment for robust global descriptors. Our overlap-based data mining and guided-triplet loss overcome the limitations of traditional distance-based mining and discrete class constraints. HeLiOS is validated on public datasets, demonstrating performance in heterogeneous LiDAR place recognition while including an evaluation for long-term recognition, showcasing its ability to handle unseen LiDAR types. We release the HeLiOS code as an open source for the robotics community at https://github.com/minwoo0611/HeLiOS.

==> fig_diff_fov_result.tex <==
\begin{figure*}[!t]
\begin{minipage}{.67\textwidth} %
  \centering
  \subfigure[Error Measured for Rotation (\textdegree) and Translation (\cm) Variation]{%
  \resizebox{0.92\textwidth}{!}{
  \begin{tabular}{c|cccc|c|ccccc}
    \toprule[1.5pt] % <-- Toprule here
    \midrule[0.5pt]
    Fixed & \multicolumn{4}{c|}{Rotation Variation (\textdegree)} &  Fixed & \multicolumn{5}{c} {Distance Variation (\cm)} \\
    Distance & 0$\rightarrow$20 & 20$\rightarrow$40 & 40$\rightarrow$60 & 60$\rightarrow$80 & Angle & 20$\rightarrow$25 & 25$\rightarrow$30 & 30$\rightarrow$35 & 35$\rightarrow$40 & 40$\rightarrow$45
    \\ \midrule[1pt]
    \unit{45}{cm} & 0.6398  & 0.0707 & 0.9675 & 1.2077 & 80\textdegree & 0.1697 & 0.1137 & 1.3918 &0.6780 & 1.3741 \\
    \unit{40}{cm} & 0.7586  & 0.1131 & 0.3187 & 0.2768 & 60\textdegree & 0.1584 & 1.0096 & 1.1799 & 1.3456 & 0.4132 \\
    \unit{35}{cm} & 0.1203  & 0.4511 & 0.8060 & 0.1947 & 40\textdegree & 0.3156 & 0.1831 & 0.7042 & 0.6292 & 0.5332 \\
    \unit{30}{cm} & 0.3974 & 0.2406 & 0.2435 & 0.3669 & 20\textdegree & 0.0120 & 0.0093 &0.3852 & 0.1017 & 0.1975 \\
    \unit{25}{cm} & 0.1790  & 0.1944 & 0.4898 & 0.1901 &  0\textdegree & 0.2690 & 0.2260 & 0.1161 & 0.1105 & 0.0595
    
    \\
    \unit{20}{cm} & 0.4953  & 0.4800 & 0.4810 & 1.1286 & & & & & & \\
   \midrule[0.5pt]
   \bottomrule[1pt]
   \end{tabular}
  }%resize 
}
  
\end{minipage}%
\begin{minipage}{.37\textwidth} %
  \centering
  \subfigure[Error Heatmap]{%
    \includegraphics[height=0.12\textheight,width=0.9\columnwidth]{figure/heatmap.pdf}
    \label{fig:heatmap}
  }
\end{minipage}
\caption{Discrepancies between estimated pose variance and its actual value. As rotation and translation trend toward the top-right quadrant of the heatmap, error rates escalate. This elevation in error is primarily ascribed to a diminishing count of diverse feature matches as both cameras progressively capture different viewpoints.}
\label{fig:diff_fov}
\vspace{-0.3cm}
\end{figure*}


==> note.tex <==
# Free Notes


% %FIGURE
% \begin{figure}[!t]
%     \centering
%    % \vspace{-1mm}
%     \subfloat[Overlap of two images\label{fig:feature_overlap1}]{
% 		\includegraphics[height=0.48\columnwidth]{./figs/overlap.png}
%     }
%     \subfloat[Revloution scan delay\label{fig:feature_overlap2}]{
% 		\includegraphics[height=0.48\columnwidth]{./figs/overlap2.png}
% 	}\\
%     \subfloat[Contour and nearest point extraction\label{fig:feature_contour}]{
% 		\includegraphics[width=0.98\columnwidth]{./figs/features.pdf}
% 	}
%     \vspace{-1mm}
%     \caption{(a) In our dataset, certain regions remain un-updated due to the low update rate. An accumulation in these overlapping areas could lead to unexpected convergence behaviors. (b) Given that radar imagery inherently constitutes scan-rotated images, there exists a discrepancy between the commencement and conclusion of the scans, primarily attributed to temporal lags. This discrepancy is especially pronounced during sharp rotational movements. (c) Initially, we delineate the contour, subsequently identifying proximal points to ensure consideration extends beyond just the central points.}
%     \label{fig:feature}
%     \vspace{-5mm}
% \end{figure}


% %FIGURE
% \begin{figure}[!t]
%     \centering
%    % \vspace{-1mm}
%     \includegraphics[width=0.98\columnwidth]{./figs/fig3.pdf}
%     \vspace{-1mm}
%     \caption{Concept of the LodeStar Descriptor. From the primary radar imagery, we compute a radial intensity vector for every $\theta$. Each of these vectors is subsequently integrated to constitute a column within the integrated radial intensity matrix. By iterating this process over a period of 2$\pi$, we synthesize the final descriptor.}
%     \label{fig:lodestar}
%     \vspace{-5mm}
% \end{figure}


root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-48-03_minmax/recall_rates.csv 
STHEREO-SNU, 56.73, 74.61, 80.08, 84.90
STHEREO-valley, 83.60, 96.46, 98.71, 99.36
vivid-urban, 92.22, 98.13, 99.22, 99.69
vivid-city, 92.02, 96.55, 98.17, 98.99

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-49-24_histeq/recall_rates.csv 
STHEREO-SNU, 63.02, 79.35, 84.41, 88.33
STHEREO-valley, 75.88, 89.39, 94.53, 96.14
vivid-urban, 91.91, 98.29, 98.91, 99.69
vivid-city, 89.25, 97.84, 98.78, 99.19

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-50-31_minmax_gridwise_8x8/recall_rates.csv 
STHEREO-SNU, 53.55, 75.02, 81.31, 86.69
STHEREO-valley, 50.80, 71.38, 76.85, 81.99
vivid-urban, 88.49, 96.58, 98.76, 99.53
vivid-city, 91.62, 96.08, 97.50, 98.65

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-51-45_minmax_gridwise_message_passing_8x8_mean_3/recall_rates.csv 
STHEREO-SNU, 61.80, 79.51, 85.22, 89.80
STHEREO-valley, 87.78, 97.43, 98.71, 99.04
vivid-urban, 93.78, 98.44, 99.07, 99.84
vivid-city, 92.97, 96.08, 97.57, 98.51

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-53-10_minmax_gridwise_message_passing_8x8_mean_5/recall_rates.csv 
STHEREO-SNU, 60.33, 77.80, 81.80, 87.27
STHEREO-valley, 90.03, 96.78, 98.07, 99.36
vivid-urban, 94.40, 99.22, 99.38, 99.84
vivid-city, 91.35, 96.42, 97.70, 98.65

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-54-42_minmax_gridwise_message_passing_16x16_mean_3/recall_rates.csv 
STHEREO-SNU, 65.71, 80.24, 84.33, 89.06
STHEREO-valley, 76.21, 91.00, 95.18, 96.78
vivid-urban, 92.07, 97.51, 99.07, 100.00
vivid-city, 90.40, 96.35, 97.77, 98.65

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-55-56_minmax_gridwise_message_passing_16x16_mean_5/recall_rates.csv 
STHEREO-SNU, 59.67, 77.55, 83.51, 88.24
STHEREO-valley, 76.85, 90.03, 95.50, 97.43
vivid-urban, 89.27, 97.20, 99.07, 99.84
vivid-city, 90.94, 95.47, 97.63, 98.58

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-57-11_minmax_gridwise_message_passing_16x16_mean_7/recall_rates.csv 
STHEREO-SNU, 60.90, 78.94, 84.90, 88.82
STHEREO-valley, 78.46, 93.89, 97.43, 99.36
vivid-urban, 90.82, 97.67, 99.38, 99.84
vivid-city, 90.80, 96.15, 97.90, 98.99

